A Short Tutorial on The Weisfeiler-Lehman Test And Its Variants

Graph neural networks are designed to learn functions on graphs. Typically, the relevant target functions are invariant with respect to actions by permutations. Therefore the design of some graph neural network architectures has been inspired by graph-isomorphism algorithms. The classical Weisfeiler-Lehman algorithm (WL) -- a graph-isomorphism test based on color refinement -- became relevant to the study of graph neural networks. The WL test can be generalized to a hierarchy of higher-order tests, known as $k$-WL. This hierarchy has been used to characterize the expressive power of graph neural networks, and to inspire the design of graph neural network architectures. A few variants of the WL hierarchy appear in the literature. The goal of this short note is pedagogical and practical: We explain the differences between the WL and folklore-WL formulations, with pointers to existing discussions in the literature. We illuminate the differences between the formulations by visualizing an example.

==> rebuttal.tex <==

Thank you for your comments. We address the questions by reviewer [213E] and [2C33] below:

Re [213E]:
Our work focused on explaining the difference between k-WL and k-FWL via an illustrative example, whereas Sato's survey provided a comprehensive review on the representation power of GNNs by connecting GNNs to WL algorithms and distributed local algorithms.

Re [2C33]:
The space constraint doesn't allow us to give a full description of the connections between WL and GNNs. We do however give some intuitions and summarize the papers in the literature that connect them.

Intuition: Many popular GNN variants can be viewed as message-passing algorithms. At each iteration, every node aggregates its neighbors' messages and updates its own state. Thus, the aggregation function in such GNNs can be seen as the hash function in the WL algorithms. 

Summary:
- WL as a tool to analyze expressive power of GNNs: [1] showed that many popular GNNs are less powerful than 1-WL, as their aggregation functions are not injective; [4] established the equivalence between WL and function approximation power with GNNs.
- WL to inspire designs of GNNs: inspired by 1-WL, [1] proposed Graph Isomorphic Networks with multi-layer perception (MLP) as an injective aggregation function and thus are as powerful as 1-WL; inspired by k-WL, [2] designed k-GNNs that implement message passing on a size-k node neighborhood and thus are as powerful as k-WL; inspired by 2-FWL, [3] proposed 2-order folklore GNNs that perform matrix multiplication after MLP aggregation functions, which are as powerful as 3-WL and enjoy computational efficiency. Similar architecture -- Ring GNN -- was proposed in [4]. [3] further generalized 2-order folklore GNNs to higher-order by using higher-order tensor multiplication. 
- Beyond WL: [5] and [6] used relational pooling to build GNNs that are provably stronger than 1-WL, by concatenating a one-hot encoding of the node index to the node feature, and averaging all permutations of the node index; [7] also added the node index, but relied on a permutation equivariant neural network at the output layer; [8] proposed Graph Substructure Networks to capture graph substructures by computing messages differently depending on the topological relationship between the endpoint nodes. 

[1] Xu, Keyulu, et al. "How powerful are graph neural networks?." arXiv preprint arXiv:1810.00826. 2018.

[2] Morris, Christopher, et al. "Weisfeiler and leman go neural: Higher-order graph neural networks." Proceedings of the AAAI Conference on Artificial Intelligence. Vol. 33. 2019.

[3] Maron, Haggai, et al. "Provably powerful graph networks." Advances in neural information processing systems. 2019.

[4] Chen, Zhengdao, et al. "On the equivalence between graph isomorphism testing and function approximation with gnns." Advances in Neural Information Processing Systems. 2019.

[5] Murphy, Ryan L., et al. "Relational pooling for graph representations." arXiv preprint arXiv:1903.02541. 2019.

[6] Chen, Zhengdao, et al. "Can graph neural networks count substructures?." arXiv preprint arXiv:2002.04025. 2020.

[7] Clément, Vignac, et al. "Building powerful and equivariant graph neural networks with structural message-passing." arXiv :2006.15107. 2020.

[8] Bouritsas, Giorgos, et al. "Improving graph neural network expressivity via subgraph isomorphism counting." arXiv preprint arXiv:2006.09252. 2020.
